Piecewise rotations: limit set for the non -bijective maps

We consider non-bijective piecewise rotations of the plane. These maps belong to a family introduced in previous papers by Boshernitzan and Goetz. We derive in this paper some upper bounds to the size of the limit set. This improves results of \cite{Bosh.Goet.03}.

==> figdemocasinj1.tex <==
\begin{tikzpicture}[scale=0.5]
% les plans
\draw[fill = red!30] (-3,-4)--(-3,2)--(6,-4)--(-3,-4);
\node[above right] at (-3,-4) {$\mathbf P_0$};
\draw[fill = blue!30] (-3,2)--(-3,2)--(6,2)--(6,-4);
\node[below left] at (6,2) {$\mathbf P_1$};
\draw[ultra thick,color=blue] (-3,2)--(6,-4);
% les centres 
\draw[->,thick,color = black] (0,0)--(1,1.5) ;
\node[right] at (1,1.5) {$C_0$};
\draw[->,thick,color = black] (3,-2)--(4.5,0.25) ; 
\node[above] at (4.5,0.25) {$C_1$}; 

\node[below] at (0,0) {$C_0'$}; 
\node[below] at (3,-2) {$C_1'$}; 

% applications
\node at (8,0) {$\longrightarrow$};
\end{tikzpicture}

==> figdemocasinj2.tex <==
\begin{tikzpicture}[scale=0.5]
% boite
\draw (-3,2)--(6,2)--(6,-4)--(-3,-4)--(-3,2);
% les plans
\draw[fill=red!30] (-1.69,2)--(-3,2)--(-3,-4)--(3.05,-4);
\draw[color=black] (-1.69,2)--(3.05,-4);
\draw[fill=blue!30] (-0.33,2)--(6,2)--(6,-4)--(4.41,-4);
\draw[ultra thick,color=blue] (-0.33,2)--(4.41,-4);
\node[below left] at (6,2) {$T(\mathbf P_1)$};
\node[above right] at (-3,-4) {$T(\mathbf P_0)$};
% les centres 
\draw[->,thick,color = black] (-0.41,0.38)--(1,1.5) ;
\node[right] at (1,1.5) {$C_0$};
\draw[->,thick,color = black] (2.38,-1.43)--(4.5,0.25) ; 
\node[above] at (4.5,0.25) {$C_1$}; 
%\node[left] at (-0.41,0.38) {$r_0(C_0')$};
%\node[right] at (2.38,-1.43) {$r_1(C_1')$};

%DELTA
\draw[<->,thick] (0.91,0.42)--(0.07,-0.24);
\node[below right] at (0,0.1) {\small $-2\Delta$};
\end{tikzpicture}


==> figdemocassurj1.tex <==
\begin{tikzpicture}[scale=0.5]
% les plans
\draw[fill = red!30] (-3,-4)--(-3,2)--(6,-4)--(-3,-4);
\node[above right] at (-3,-4) {$\mathbf P_0$};
\draw[fill = blue!30] (-3,2)--(-3,2)--(6,2)--(6,-4);
\node[below left] at (6,2) {$\mathbf P_1$};
\draw[ultra thick,color=blue] (-3,2)--(6,-4);
% les centres 
\draw[->,thick,color = black] (0,0)--(1,1.5) ;
\node[right] at (1,1.5) {$C_0$};
\draw[->,thick,color = black] (3,-2)--(4.5,0.25) ; 
\node[above] at (4.5,0.25) {$C_1$}; 

\node[below] at (0,0) {$C_0'$}; 
\node[below] at (3,-2) {$C_1'$}; 

% applications
\node at (8,0) {$\longrightarrow$};
\end{tikzpicture}

==> figdemocassurj2.tex <==
\begin{tikzpicture}[scale=0.5]
% boite
\draw (-3,2)--(6,2)--(6,-4)--(-3,-4)--(-3,2);
% les plans
\draw[fill=red!30] (-3,0.75)--(-3,-4)--(6,-4)--(6,-1.77);
\draw[fill=blue!30,opacity=0.6] (-3,-0.45)--(-3,2)--(6,2)--(6,-2.98);
\draw[ultra thick,color=blue] (-3,-0.45)--(6,-2.98);
\draw[color=black] (-3,0.75)--(6,-1.77);
\node[below left] at (6,2) {$T(\mathbf P_1)$};
\node[above right] at (-3,-4) {$T(\mathbf P_0)$};
% les centres 
\draw[->,thick,color = black] (0.51,-0.24) --(1,1.5) ;
\node[right] at (1,1.5) {$C_0$};
\draw[->,thick,color = black] (3.77,-2.35)--(4.5,0.25) ; 
\node[above] at (4.5,0.25) {$C_1$}; 
%\node[right] at (0.51,-0.24) {$r_0(C_0')$};
%\node[below] at (3.77,-2.35){$r_1(C_1')$};

% DELTA
\draw[<->] (1.09,-1.60) -- (1.40,-0.49);
\node[right] at (1.2,-1.1) {\small $2\Delta$}; 
\end{tikzpicture} 
 

==> figespacephases.tex <==
\begin{tikzpicture}

\node[below] at (-2,-2) {$-\pi$};
\node[below] at (-1,-2) {$-\frac\pi2$};
\node[below] at (0,-2) {$0$};
\node[below] at (1,-2) {$\frac\pi2$};
\node[below] at (2,-2) {$\pi$};

\node[left] at (-2,-2) {$-\pi$};
\node[left] at (-2,-1) {$-\frac\pi2$};
\node[left] at (-2,0) {$0$};
\node[left] at (-2,1) {$\frac\pi2$};
\node[left] at (-2,2) {$\pi$};

\draw[fill = blue!30] (-2,1)--(-2,2)--(0,2);
\draw[fill = blue!30] (-2,-1)--(-2,-2)--(0,-2)--(0,0);
\draw[fill = blue!30] (2,-1)--(2,-2)--(0,-2);
\draw[fill = blue!30] (2,1)--(2,2)--(0,2)--(0,0);

\draw[fill = green!30] (-2,-1)--(-2,1)--(0,2)--(0,0);
\draw[fill = green!30] (2,1)--(2,-1)--(0,-2)--(0,0);

\draw[-,color = red,ultra thick] (-2,1)--(0,2);
\draw[-,color = red,ultra thick] (-2,-1)--(2,1);
\draw[-,color = red,ultra thick] (0,-2)--(2,-1);

\draw (0,-2)--(2.5,-2);
\node[below] at (2.5,-2) {$\alpha$};

\draw (-2,0)--(-2,2.5);
\node[left] at (-2,2.5) {$\beta$};

\draw[-,thick] (-2,-2)--(-2,2)--(2,2)--(2,-2)--(-2,-2);
\draw[-,thick] (0,-2)--(0,2);
\draw[-,thick] (-2,0)--(2,0);




%Legende
\draw[-,thick,fill = green!30] (3,1.5)--(3,2)--(4,2)--(4,1.5)--(3,1.5);
\node[right] at (4.2,1.75) {surjective and non-injective};
\draw[-,thick,fill = blue!30] (3,1)--(3,1.5)--(4,1.5)--(4,1)--(3,1);
\node[right] at (4.2,1.25) {injective and non-surjective};
\draw[-,ultra thick,color = red] (3,0.75)--(4,0.75);
\node[right] at (4.2,0.75) {invertible};


\end{tikzpicture}
 
